Studies of the resonance structure in $D^{0} \to K^\mp \pi^\pm \pi^\pm \pi^\mp$ decays

Amplitude models are constructed to describe the resonance structure of ${D^{0}\to K^{-}\pi^{+}\pi^{+}\pi^{-}}$ and ${D^{0} \to K^{+}\pi^{-}\pi^{-}\pi^{+}}$ decays using $pp$ collision data collected at centre-of-mass energies of 7 and 8 TeV with the LHCb experiment, corresponding to an integrated luminosity of $3.0\mathrm{fb}^{-1}$. The largest contributions to both decay amplitudes are found to come from axial resonances, with decay modes $D^{0} \to a_1(1260)^{+} K^{-}$ and $D^{0} \to K_1(1270/1400)^{+} \pi^{-}$ being prominent in ${D^{0}\to K^{-}\pi^{+}\pi^{+}\pi^{-}}$ and $D^{0}\to K^{+}\pi^{-}\pi^{-}\pi^{+}$, respectively. Precise measurements of the lineshape parameters and couplings of the $a_1(1260)^{+}$, $K_1(1270)^{-}$ and $K(1460)^{-}$ resonances are made, and a quasi model-independent study of the $K(1460)^{-}$ resonance is performed. The coherence factor of the decays is calculated from the amplitude models to be $R_{K3\pi} = 0.459\pm 0.010\,(\mathrm{stat}) \pm 0.012\,(\mathrm{syst}) \pm 0.020\,(\mathrm{model})$, which is consistent with direct measurements. These models will be useful in future measurements of the unitary-triangle angle $\gamma$ and studies of charm mixing and $C\!P$ violation.

==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN   = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count* 
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated 
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prlNotes.bib

# remove output file
rmout: 
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl: 
	$(BUILDCOMMANDPRL)

# Make the PRL version
count: 
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo 


==> tables/RS_w1450/FitFractionModelChoice.tex <==
\begin{tabular}{l 
>{\collectcell\num}r<{\endcollectcell} @{${}\pm{}$} >{\collectcell\num}l<{\endcollectcell} @{${}\pm{}$} >{\collectcell\num}r<{\endcollectcell}
>{\collectcell\num}r<{\endcollectcell} @{${}\pm{}$} >{\collectcell\num}l<{\endcollectcell}
}
\toprule
 & \multicolumn{5}{c}{(Partial) Fraction [\%]}\\
  & \multicolumn{3}{c}{Baseline} & \multicolumn{2}{c}{Ensemble} \\
  & \multicolumn{3}{c}{} & \multicolumn{1}{r}{Mean} & \multicolumn{1}{l}{\!RMS} \\
\midrule
  $\left[\Kstarb(892)^{0}\rho(770)^{0}\right]^{L=0}$                                                 & 7.34  & 0.08 & 0.47 & 7.10  & 0.13\\
  $\left[\Kstarb(892)^{0}\rho(770)^{0}\right]^{L=1}$                              & 6.03  & 0.05 & 0.25 & 6.00  & 0.12\\
  $\left[\Kstarb(892)^{0}\rho(770)^{0}\right]^{L=2}$                              & 8.47  & 0.09 & 0.67 & 8.42  & 0.20\\
  $\left[\rho(1450)^{0}\Kstarb(892)^{0}\right]^{L=0}$                                                & 0.61  & 0.04 & 0.17 & 0.65  & 0.13\\
  $\left[\rho(1450)^{0}\Kstarb(892)^{0}\right]^{L=1}$                             & 1.98  & 0.03 & 0.33 & 1.91  & 0.06\\
  $\left[\rho(1450)^{0}\Kstarb(892)^{0}\right]^{L=2}$                             & 0.46  & 0.03 & 0.15 & 0.46  & 0.05\\
\midrule
  $\rho(770)^{0}\left[\Km\pip\right]^{L=0}$                              & 0.93  & 0.03 & 0.05 & 1.08  & 0.12\\
  $\Kstarb(892)^{0}\left[\pi^{+}\pi^{-}\right]^{L=0}$                             & 2.35  & 0.09 & 0.33 & 2.19  & 0.34\\
\midrule
  $a_{1}(1260)^{+}K^{-}$                                             & 38.07 & 0.24 & 1.38 & 38.06 & 2.08\\
  $\quad \rho(770)^{0}\pi^{+}$                                                         & 89.75 & 0.45 & 1.00 & 86.66 & 4.52\\
  $\quad \left[\pi^{+}\pi^{-}\right]^{L=0}\pi^{+}$                                     & 2.42  & 0.06 & 0.12 & 3.01 & 1.02\\
  $\quad \left[\rho(770)^{0}\pi^{+}\right]^{L=2}$                                      & 0.85  & 0.03 & 0.06 & 0.80 & 0.10\\
  $K_{1}(1270)^{-}\pi^{+}$                                                    & 4.66  & 0.05 & 0.39 & 4.74 & 0.24\\
  $\quad \rho(770)^{0}K^{-}$                                                  & 96.30 & 1.64 & 6.61 & 77.04 & 9.22\\
  $\quad \rho(1450)^{0}K^{-}$                                                 & 49.09 & 1.58 & 11.54& 34.13 & 8.19\\
  $\quad \omega(782)\left[\pi^{+}\pi^{-}\right]K^{-}$                         & 1.65  & 0.11 & 0.16 & 1.70 & 0.15\\
  $\quad \Kstarb(892)^{0}\pi^{-}$                                                 & 27.08 & 0.64 & 2.82 & 26.95 & 2.52\\
  $\quad \left[\Kstarb(892)^{0}\pi^{-}\right]^{L=2}$                              & 3.47  & 0.17 & 0.31 & 3.57 & 0.49\\
  $\quad \left[K^{-}\pi^{+}\right]\pi^{-}$                                    & 22.90 & 0.72 & 1.89  & 20.39 & 2.89\\
  $K_{1}(1400)^{-}\left[\Kstarb(892)^{0}\pi^{-}\right]\pi^{+}$           & 1.15  & 0.04 & 0.20 & 1.23 & 0.10\\
\midrule
  $K_{2}^{*}(1430)^{-}\left[\Kstarb(892)^{0}\pi^{-}\right]\pi^{+}$       & 0.46 & 0.01 & 0.03 & 0.44 & 0.04\\
\midrule
  $K(1460)^{-}\pi^{+}$                                                        & 3.75 & 0.10 & 0.37 & 3.63 & 0.27\\
  $\quad \Kstarb(892)^{0}\pi^{-}$                                                 & 51.39 & 1.00 & 1.71 & 53.18 & 1.52\\
  $\quad \left[\pi^{+}\pi^{-}\right]^{L=0}K^{-}$                              & 31.23 & 0.83 & 1.78 & 30.46 & 1.19\\
\midrule
  $\left[\Km\pi^{+}\right]^{L=0}\left[\pi^{+}\pi^{-}\right]^{L=0}$            & 22.04 & 0.28 & 2.09 & 21.87 & 1.51\\
\bottomrule
\end{tabular}


==> tables/RS_w1450/InterferenceFractions.tex <==
\begin{tabular}{l l 
>{\collectcell\num}r<{\endcollectcell} @{${}\pm{}$} >{\collectcell\num}l<{\endcollectcell} @{${}\pm{}$} >{\collectcell\num}l<{\endcollectcell}
}
\toprule
  Decay chain $a$ & Decay chain $b$ & \multicolumn{3}{c}{Interference Fraction $\left[\%\right]$} \\
\midrule
$\Kstarb(892)^{0}\rho(770)^{0}  $&$ {a}_{1}(1260)^{+}{K}^{-}$ & 5.74  & 0.03  & 0.1 \\
$\left[\Kstarb(892)^{0}\rho(770)^{0}\right]^{L=2} $&$ \Kstarb(892)^{0}\rho(770)^{0}$  & -2.59 & 0.02  & 0.07  \\
$\left[{K}^{+}\pi^{-}\right]^{L=0}\left[\pi^{+}\pi^{-}\right]^{L=0} $&$ {a}_{1}(1260)^{+}{K}^{-}$ & 2.4 & 0.03  & 0.14  \\
${a}_{1}(1260)^{+}{K}^{-} $&$ \rho(770)^{0}\left[{K}^{-}\pi^{+}\right]^{L=0}$ & 2.14  & 0.07  & 0.26  \\
$\left[\Kstarb(892)^{0}\rho(770)^{0}\right]^{L=2} $&$ {a}_{1}(1260)^{+}{K}^{-}$ & -1.76 & 0.01  & 0.08  \\
$\left[\Kstarb(892)^{0}\rho(770)^{0}\right]^{L=1} $&$ \left[\rho(1450)^{0}\Kstarb(892)^{0}\right]^{L=1}$  & -1.55 & 0.02  & 0.18  \\
${K}_{1}(1270)^{-}\pi^{+} $&$ \Kstarb(892)^{0}\rho(770)^{0}$  & -1.05 & 0.02  & 0.14  \\
${K}_{1}(1400)^{-}\left[\Kstarb(892)^{0}\pi^{-}\right]\pi^{+} $&$ \Kstarb(892)^{0}\rho(770)^{0}$ & 0.96  & 0.02  & 0.1 \\
$\Kstarb(892)^{0}\rho(770)^{0}  $&$ \rho(1450)^{0}\Kstarb(892)^{0}$ & -0.83 & 0.05  & 0.11  \\
$\left[\Kstarb(892)^{0}\rho(770)^{0}\right]^{L=2} $&$ \left[\rho(1450)^{0}\Kstarb(892)^{0}\right]^{L=2}$  & 0.81  & 0.04  & 0.13  \\
${K}(1460)^{-}\pi^{+} $&$ \Kstarb(892)^{0}\left[\pi^{+}\pi^{-}\right]^{L=0}$  & 0.78  & 0.03  & 0.1 \\
$\Kstarb(892)^{0}\rho(770)^{0}  $&$ \left[\Km\pip\right]^{L=0}\left[\pi^{+}\pi^{-}\right]^{L=0}$ & 0.73  & 0.01  & 0.03  \\
$\Kstarb(892)^{0}\left[\pi^{+}\pi^{-}\right]^{L=0}  $&$ {a}_{1}(1260)^{+}{K}^{-}$ & -0.68 & 0.01  & 0.07  \\
${K}_{1}(1270)^{-}\pi^{+} $&$ {K}_{1}(1400)^{-}\left[\Kstarb(892)^{0}\pi^{-}\right]\pi^{+}$ & -0.67 & 0.02  & 0.12  \\
${K}(1460)^{-}\pi^{+} $&$ \Kstarb(892)^{0}\rho(770)^{0}$  & -0.66 & 0.02  & 0.05  \\
${a}_{1}(1260)^{+}{K}^{-} $&$ \rho(1450)^{0}\Kstarb(892)^{0}$ & -0.63 & 0.02  & 0.08  \\
$\left[\Kstarb(892)^{0}\rho(770)^{0}\right]^{L=2} $&$ {K}(1460)^{-}\pi^{+}$ & -0.6  & 0.02  & 0.07  \\
${K}(1460)^{-}\pi^{+} $&$ \rho(1450)^{0}\Kstarb(892)^{0}$ & 0.51  & 0.01  & 0.06  \\
\bottomrule
\end{tabular}


==> tables/RS_w1450/ModelSummary.tex <==
\begin{tabular}{l 
r 
r 
}
\toprule
Mode & Fraction & $\langle \mathcal{F} \rangle$\\
 & of models $[\%]$ & $[\%]$\\
\midrule
$K_{1}(1400)^{-}\left[\rho(1450)^{0}K^{-}\right]\pi^{+}$ & 13.6 & 0.319\\
$K(1460)^{-}\left[K_{2}^{*}(1430)^{0}\pi^{-}\right]\pi^{+}$ & 13.1 & 0.060\\
$K^{*}(1680)^{-}\left[\rho(770)^{0}K^{-}\right]\pi^{+}$ & 13.1 & 0.068\\
$K_{2}^{*}(1430)^{-}\left[\rho(1450)^{0}K^{-}\right]\pi^{+}$ & 13.1 & 0.096\\
$K_{2}^{*}(1430)^{-}\left[K^*(1680)^{0}\pi^{-}\right]\pi^{+}$ & 13.1 & 0.133\\
$K_{2}^{*}(1430)^{-}\left[K^*(1410)^{0}\pi^{-}\right]\pi^{+}$ & 13.1 & 0.123\\
$K_{1}(1400)^{-}\left[\rho(770)^{0}K^{-}\right]\pi^{+}$ & 13.1 & 0.449\\
$K_{1}(1400)^{-}\left[K^*(1410)^{0}\pi^{-}\right]\pi^{+}$ & 13.1 & 0.112\\
$a_{1}(1640)^{+}\left[\left[\pi^+\pi^-\right]^{L=0}\pi^{+}\right]K^{-}$ & 12.1 & 2.468\\
\bottomrule
\end{tabular}


==> tables/WS_w1450/BinnedCoherence.tex <==
\begin{tabular}{l 
>{\collectcell\num}r<{\endcollectcell} @{${}\pm{}$} >{\collectcell\num}l<{\endcollectcell}
>{\collectcell\num}r<{\endcollectcell} @{${}\pm{}$} >{\collectcell\num}l<{\endcollectcell}
>{\collectcell\num}r<{\endcollectcell} @{${}\pm{}$} >{\collectcell\num}l<{\endcollectcell}
}
\toprule
Bin & \multicolumn{2}{c}{$R_{K3\pi}$} & \multicolumn{2}{c}{$\delta_{K3\pi} [^o]$} & \multicolumn{2}{c}{$r_{K3\pi} \times 10^{-2}$}\\
\midrule
Global & 0.471 & 0.040 & \multicolumn{2}{c}{128} & \multicolumn{2}{c}{5.49}\\
\midrule
1 & 0.481 & 0.019 & -103 & 10 & 4.364 & 0.088\\
2 & 0.723 & 0.017 & -143 & 4 & 5.121 & 0.047\\
3 & 0.721 & 0.019 & -161 & 2 & 5.669 & 0.073\\
4 & 0.743 & 0.017 & -158 & 81 & 6.149 & 0.074\\
5 & 0.767 & 0.014 & 167 & 2 & 6.204 & 0.066\\
6 & 0.789 & 0.011 & 152 & 3 & 6.061 & 0.056\\
7 & 0.751 & 0.009 & 135 & 3 & 5.792 & 0.055\\
8 & 0.417 & 0.012 & 78 & 6 & 5.537 & 0.097\\
\bottomrule
\end{tabular}


==> tables/WS_w1450/fractions_systematics_table.tex <==
\begin{tabular}{l 
>{\collectcell\num}r<{\endcollectcell} @{${}\pm{}$} >{\collectcell\num}l<{\endcollectcell} @{${}\pm{}$} >{\collectcell\num}l<{\endcollectcell}
l 
l 
l 
l 
l 
l 
}
\toprule
 & \multicolumn{3}{c}{Fit Fraction [\%]} & \multicolumn{1}{c}{II} & \multicolumn{1}{c}{III} & \multicolumn{1}{c}{IV} & \multicolumn{1}{c}{V} & \multicolumn{1}{c}{VI} & \multicolumn{1}{c}{VII}\\
\midrule
\midrule
\midrule
$K_{1}(1400)^{+}\left[K^*(892)^{0}\pi^{+}\right]\pi^{-}$ & 26.549 & 1.973 & 2.128 & 0.190 & 1.715 & 0.469 & 0.046 & 0.940 & 0.667\\
\midrule
\bottomrule
\end{tabular}


==> tables/WS_w1450/systematics_table.tex <==
\begin{tabular}{l 
l 
>{\collectcell\num}r<{\endcollectcell} @{${}\pm{}$} >{\collectcell\num}l<{\endcollectcell} @{${}\pm{}$} >{\collectcell\num}l<{\endcollectcell}
l 
l 
l 
l 
l 
l 
}
\toprule
 &  & \multicolumn{3}{c}{} & \multicolumn{1}{c}{II} & \multicolumn{1}{c}{III} & \multicolumn{1}{c}{IV} & \multicolumn{1}{c}{V} & \multicolumn{1}{c}{VI} & \multicolumn{1}{c}{VII}\\
\midrule
\multirow{2}{*}{$K^*(892)^{0}\rho(770)^{0}$} & $\left| g \right|$ & 0.205 & 0.019 & 0.010 & 0.002 & 0.006 & 0.003 & 0.001 & 0.005 & 0.006\\
 & $\mathrm{arg}(g) [^o]$ & -8.502 & 4.662 & 4.439 & 0.433 & 1.272 & 0.112 & 0.148 & 4.150 & 0.799\\
 & $\mathcal{F}$ & 9.617 & 1.584 & 1.028 & 0.134 & 0.436 & 0.344 & 0.069 & 0.567 & 0.637\\
  
\multirow{3}{*}{$\left[K^*(892)^{0}\rho(770)^{0}\right]^{L=1}$} & $\left| g \right|$ & 0.390 & 0.029 & 0.006 & 0.002 & 0.003 & 0.000 & 0.001 & 0.004 & 0.003\\
 & $\mathrm{arg}(g) [^o]$ & -91.359 & 4.728 & 4.132 & 0.406 & 0.827 & 0.128 & 0.101 & 3.951 & 0.766\\
 & $\mathcal{F}$ & 8.424 & 0.827 & 0.573 & 0.069 & 0.091 & 0.210 & 0.020 & 0.458 & 0.249\\

  
 $\left[K^*(892)^{0}\rho(770)^{0}\right]^{L=2}$ & $\mathcal{F}$ & 10.191 & 1.028 & 0.789 & 0.089 & 0.130 & 0.255 & 0.018 & 0.658 & 0.314\\
  \multirow{3}{*}{$\rho(1450)^{0}K^*(892)^{0}$} & $\left| g \right|$ & 0.541 & 0.042 & 0.055 & 0.004 & 0.043 & 0.018 & 0.001 & 0.024 & 0.016\\
 & $\mathrm{arg}(g) [^o]$ & -21.798 & 6.536 & 5.483 & 0.573 & 4.532 & 0.547 & 0.254 & 0.254 & 2.960\\
  & $\mathcal{F}$ & 8.162 & 1.242 & 1.686 & 0.107 & 1.381 & 0.474 & 0.031 & 0.718 & 0.428\\
\midrule
\multirow{2}{*}{$K_{1}(1270)^{+}\pi^{-}$} & $\left| g \right|$ & 0.653 & 0.040 & 0.058 & 0.004 & 0.017 & 0.009 & 0.001 & 0.049 & 0.024\\
 & $\mathrm{arg}(g) [^o]$ & -110.715 & 5.054 & 4.854 & 0.481 & 1.484 & 0.219 & 0.056 & 4.236 & 1.770\\
 & $\mathcal{F}$ & 18.147 & 1.114 & 2.301 & 0.104 & 0.800 & 0.423 & 0.021 & 1.788 & 1.125\\
\multirow{2}{*}{$K_{1}(1400)^{+}\left[K^*(892)^{0}\pi^{+}\right]\pi^{-}$} & $\left| g \right|$ & 0.560 & 0.037 & 0.031 & 0.003 & 0.020 & 0.011 & 0.001 & 0.018 & 0.010\\
 & $\mathrm{arg}(g) [^o]$ & 29.769 & 4.220 & 4.565 & 0.396 & 4.055 & 0.211 & 0.060 & 1.638 & 1.227\\
 & $\mathcal{F}$ & 26.549 & 1.973 & 2.128 & 0.190 & 1.715 & 0.469 & 0.046 & 0.940 & 0.667\\
\midrule
  $\left[K^{+}\pi^{-}\right]^{L=0}\left[\pi^{+}\pi^{-}\right]^{L=0}$ & $\mathcal{F}$ & 20.901 & 1.295 & 1.500 & 0.129 & 0.328 & 0.565 & 0.134 & 1.246 & 0.486\\
\multirow{2}{*}{$\quad \alpha_{3/2}$} & $\left| g \right|$ & 0.686 & 0.043 & 0.022 & 0.004 & 0.007 & 0.002 & 0.002 & 0.019 & 0.007\\
 & $\mathrm{arg}(g) [^o]$ & -149.399 & 4.260 & 2.946 & 0.502 & 0.277 & 0.181 & 0.082 & 2.809 & 0.651\\
\multirow{2}{*}{$\quad \beta_1$} & $\left| g \right|$ & 0.438 & 0.044 & 0.030 & 0.004 & 0.006 & 0.010 & 0.001 & 0.026 & 0.010\\
 & $\mathrm{arg}(g) [^o]$ & -132.424 & 6.507 & 2.972 & 0.618 & 1.109 & 0.357 & 0.200 & 2.382 & 1.174\\
\multirow{2}{*}{$\quad f_{\pi\pi}$} & $\left| g \right|$ & 0.050 & 0.006 & 0.005 & 0.001 & 0.001 & 0.001 & 0.000 & 0.004 & 0.002\\
 & $\mathrm{arg}(g) [^o]$ & 74.821 & 7.528 & 5.282 & 0.695 & 0.745 & 0.149 & 0.472 & 5.050 & 1.058\\
\bottomrule
\end{tabular}


==> tables/systematics_table.tex <==
\begin{tabular}{l 
l 
>{\collectcell\num}r<{\endcollectcell} @{${}\pm{}$} >{\collectcell\num}l<{\endcollectcell} @{${}\pm{}$} >{\collectcell\num}l<{\endcollectcell}
l 
l 
l 
l 
l 
}
\toprule
 &  & \multicolumn{3}{c}{} & \multicolumn{1}{c}{I} & \multicolumn{1}{c}{II} & \multicolumn{1}{c}{III} & \multicolumn{1}{c}{IV} & \multicolumn{1}{c}{V}\\
\midrule
$\Kstarb(892)^{0}\rho(770)^{0}$ & $\mathcal{F}$ & 7.340 & 0.084 & 0.637 & 0.426 & 0.050 & 0.063 & 0.466 & 0.025\\
 & $\left| g \right|$ & 0.196 & 0.001 & 0.015 & 0.000 & 0.001 & 0.001 & 0.015 & 0.000\\
 & $arg(g) [^o]$ & -22.363 & 0.361 & 1.644 & 1.309 & 0.239 & 0.119 & 0.955 & 0.075\\
$\left[\Kstarb(892)^{0}\rho(770)^{0}\right]^{L=1}$ & $\mathcal{F}$ & 6.031 & 0.049 & 0.436 & 0.358 & 0.029 & 0.061 & 0.239 & 0.006\\
 & $\left| g \right|$ & 0.362 & 0.002 & 0.010 & 0.002 & 0.001 & 0.002 & 0.009 & 0.000\\
 & $arg(g) [^o]$ & -102.907 & 0.380 & 1.667 & 1.431 & 0.224 & 0.321 & 0.760 & 0.025\\
$\left[\Kstarb(892)^{0}\rho(770)^{0}\right]^{L=2}$ & $\mathcal{F}$ & 8.475 & 0.086 & 0.826 & 0.492 & 0.051 & 0.059 & 0.659 & 0.023\\
$\rho(1450)^{0}\Kstarb(892)^{0}$ & $\mathcal{F}$ & 0.608 & 0.040 & 0.165 & 0.061 & 0.032 & 0.134 & 0.065 & 0.019\\
 & $\left| g \right|$ & 0.162 & 0.005 & 0.025 & 0.007 & 0.004 & 0.018 & 0.015 & 0.003\\
 & $arg(g) [^o]$ & -86.122 & 1.852 & 4.345 & 1.933 & 1.570 & 2.485 & 2.152 & 1.368\\
$\left[\rho(1450)^{0}\Kstarb(892)^{0}\right]^{L=1}$ & $\mathcal{F}$ & 1.975 & 0.029 & 0.351 & 0.115 & 0.017 & 0.315 & 0.103 & 0.003\\
 & $\left| g \right|$ & 0.643 & 0.006 & 0.058 & 0.001 & 0.003 & 0.050 & 0.029 & 0.001\\
 & $arg(g) [^o]$ & 97.304 & 0.516 & 2.770 & 2.249 & 0.288 & 1.341 & 0.854 & 0.031\\
$\left[\rho(1450)^{0}\Kstarb(892)^{0}\right]^{L=2}$ & $\mathcal{F}$ & 0.455 & 0.028 & 0.163 & 0.078 & 0.016 & 0.090 & 0.110 & 0.004\\
 & $\left| g \right|$ & 0.649 & 0.021 & 0.105 & 0.052 & 0.011 & 0.063 & 0.065 & 0.003\\
 & $arg(g) [^o]$ & -15.564 & 1.960 & 4.109 & 1.208 & 1.323 & 2.631 & 2.484 & 0.762\\
\midrule
$\rho(770)^{0}\left[K^{-}\pi^{+}\right]^{L=0}$ & $\mathcal{F}$ & 0.926 & 0.032 & 0.083 & 0.069 & 0.019 & 0.016 & 0.039 & 0.006\\
 & $\left| g \right|$ & 0.338 & 0.006 & 0.011 & 0.000 & 0.004 & 0.002 & 0.010 & 0.002\\
 & $arg(g) [^o]$ & 73.048 & 0.795 & 3.951 & 3.567 & 0.469 & 0.481 & 1.549 & 0.185\\
$\quad \alpha_{3/2}$ & $\left| g \right|$ & 1.073 & 0.008 & 0.021 & 0.018 & 0.005 & 0.005 & 0.009 & 0.003\\
 & $arg(g) [^o]$ & -130.856 & 0.457 & 1.786 & 1.679 & 0.282 & 0.274 & 0.435 & 0.155\\
$\Kstarb(892)^{0}\left[\pi^{+}\pi^{-}\right]^{L=0}$ & $\mathcal{F}$ & 2.347 & 0.089 & 0.557 & 0.483 & 0.079 & 0.148 & 0.206 & 0.076\\
$\quad f_{\pi\pi}$ & $\left| g \right|$ & 0.261 & 0.005 & 0.024 & 0.022 & 0.004 & 0.006 & 0.007 & 0.003\\
 & $arg(g) [^o]$ & -149.023 & 0.943 & 2.696 & 2.275 & 0.540 & 1.176 & 0.617 & 0.196\\
$\quad \beta_1$ & $\left| g \right|$ & 0.305 & 0.011 & 0.046 & 0.040 & 0.010 & 0.013 & 0.013 & 0.007\\
 & $arg(g) [^o]$ & 65.554 & 1.534 & 4.004 & 3.017 & 0.857 & 2.322 & 0.771 & 0.455\\
\midrule
$\left[K^{-}\pi^{+}\right]^{L=0}\left[\pi^{+}\pi^{-}\right]^{L=0}$ & $\mathcal{F}$ & 22.044 & 0.282 & 4.137 & 3.631 & 0.268 & 0.213 & 1.945 & 0.188\\
$\quad \alpha_{3/2}$ & $\left| g \right|$ & 0.870 & 0.010 & 0.030 & 0.029 & 0.005 & 0.003 & 0.004 & 0.002\\
 & $arg(g) [^o]$ & -149.187 & 0.712 & 3.503 & 3.467 & 0.350 & 0.250 & 0.194 & 0.157\\
$\quad \alpha_{K\eta^\prime}$ & $\left| g \right|$ & 2.614 & 0.141 & 0.281 & 0.263 & 0.063 & 0.041 & 0.062 & 0.018\\
 & $arg(g) [^o]$ & -19.073 & 2.414 & 11.979 & 11.775 & 1.507 & 1.151 & 0.816 & 0.755\\
$\quad \beta_1$ & $\left| g \right|$ & 0.554 & 0.009 & 0.053 & 0.019 & 0.005 & 0.004 & 0.050 & 0.002\\
 & $arg(g) [^o]$ & 35.310 & 0.662 & 1.627 & 0.969 & 0.439 & 0.588 & 1.069 & 0.168\\
$\quad f_{\pi\pi}$ & $\left| g \right|$ & 0.082 & 0.001 & 0.008 & 0.004 & 0.001 & 0.001 & 0.007 & 0.000\\
 & $arg(g) [^o]$ & -146.991 & 0.718 & 2.248 & 1.849 & 0.463 & 0.593 & 1.003 & 0.252\\
\bottomrule
\end{tabular}


==> tex/Discussion.tex <==

\subsection{Coherence Factor} 

\subsection{Local P-violation}

